Quantum computing for corrosion-resistant materials and anti-corrosive coatings design

Corrosion is a pervasive issue that impacts the structural integrity and performance of materials across various industries, imposing a significant economic impact globally. In fields like aerospace and defense, developing corrosion-resistant materials is critical, but progress is often hindered by the complexities of material-environment interactions. While computational methods have advanced in designing corrosion inhibitors and corrosion-resistant materials, they fall short in understanding the fundamental corrosion mechanisms due to the highly correlated nature of the systems involved. This paper explores the potential of leveraging quantum computing to accelerate the design of corrosion inhibitors and corrosion-resistant materials, with a particular focus on magnesium and niobium alloys. We investigate the quantum computing resources required for high-fidelity electronic ground-state energy estimation (GSEE), which will be used in our hybrid classical-quantum workflow. Representative computational models for magnesium and niobium alloys show that 2292 to 38598 logical qubits and $(1.04$ to $1962) \times 10^{13}$ T-gates are required for simulating the ground-state energy of these systems under the first quantization encoding using plane waves basis.

==> classical_analysis.tex <==
%% Wil merge back to the main tex when done...

\subsection{Limitations of Classical Methods for Estimating Ground-State Energies}

The solution of the electronic Schr\"{o}dinger equation to predict \emph{ab initio} properties of chemical and material systems has been a challenge for nearly a century. Within the Born-Oppenheimer approximation, the electronic Schr\"{o}dinger equation is
\begin{equation}
    \label{eq: time-independent schrodinger}
    \left( -\sum_i \left( \frac{\nabla_{r_i}^2}{2} + \sum_I \frac{Z_I}{|r_i - R_I|} \right) + \sum_{i<j} \frac{1}{|r_i - r_j|} \right) |\Psi(r;R)\rangle = E[\vec{r};R] |\Psi(r;R)\rangle
\end{equation}
where \(r\) is the electronic coordinate, \(R\) is the nuclear coordinate, and \(Z_I\) represents the nuclear charges. Solving this exactly is challenging due to the Coulomb repulsion between electrons. It is very straightforward to write down a guaranteed exact solution for \(\eta\) electrons in \(M\) spatial orbitals, but the solution of this problem scales exponentially in both memory and floating-point operations. As a result, exact solutions are currently limited to \(\eta=26\), \(M=23\) \cite{gao2024distributed}. 

A widely used and efficient method for electronic structure calculations is Density Functional Theory (DFT). The Hohenberg-Kohn theorem~\cite{Hohenberg1964Inhomogeneous} establishes a one-to-one correspondence between the ground-state electronic density and the defined Hamiltonian, effectively reducing the system’s degrees of freedom to just the density. This reduction allows DFT to scale significantly better than other methods, particularly as system size increases, with linear scaling $O(N)$ achieved in recent advancements~\cite{Nakata2020Large}, where $N$ is a generic parameter for number of basis functions used in the calculation. The efficiency of DFT has enabled large-scale calculations on systems with millions of atoms. For instance, CONQUEST, a linear-scaling DFT code, has been used to perform calculations on systems containing up to 2 million atoms, leveraging 705,024 physical cores on the Japanese Fujitsu-made K-computer~\cite{Nakata2020Large}. Similarly, DFT-FE, another large-scale DFT code utilizing high-order finite element discretization and adaptive spatial discretization strategies, has successfully simulated large-scale Mg dislocation systems, such as pyrIIScrewC with 6,164 Mg atoms (61,640 electrons) and pyrIIScrewC with 10,508 Mg atoms (105,080 electrons), using Summit GPU nodes~\cite{Das2019Fast}. However, despite its efficiency, DFT often falls short of delivering the high accuracy required for out-of-equilibrium chemical systems, which are the focus of our computational workflow. This is because, in practice, DFT approximates the exchange-correlation energy, a critical component for the method's accuracy. In other words, while DFT is exact in principle, it relies on approximations of this key quantity through exchange-correlation functionals, and no systematic approach exists to improve these approximations across all systems. The choice of functional depends on the specific chemical system being studied, and as a result, DFT can struggle to capture all the nuances of different bonding situations~\cite{Mardirossian2017Narbe}. 

While DFT is efficient and widely used, it is limited by its reliance on approximating the exchange-correlation functional, particularly in systems with strong electronic correlations. To overcome these limitations, many-electron wavefunction theories such as coupled-cluster (CC) theory provide a rigorous approach to achieve high accuracy. In the second-quantization formalism, the CC wavefunction is given by:
\begin{equation} 
\label{eq: Coupled Cluster} 
|\psi_{\text{CC}} \rangle = e^{\hat{T}}|\Phi_0\rangle = \sum_{i} \frac{1}{i!} (\hat{T})^n |\Phi_0\rangle 
\end{equation}
where \(\hat{T}\) is the cluster operator, defined as a sum of excitation operators \(\hat{T}_n\) for \(n\)-fold electron excitations:
\begin{align} 
    \hat{T} &= \hat{T}_1 + \hat{T}_2 + \dots + \hat{T}_n \\
    &= \sum_{ai} t_i^a \hat{a}^\dagger_a \hat{a}_i
    + \frac{1}{4} \sum_{abij} t_{ij}^{ab} \hat{a}^\dagger_a \hat{a}^\dagger_b \hat{a}_j \hat{a}_i
    + \cdots + \frac{1}{(n!)^2} \sum_{i_1, \cdots, i_n, a_1, \cdots, a_n} t_{i_1 \cdots i_n}^{a_1 \cdots a_n} \hat{a}_{a_1}^\dagger \cdots \hat{a}_{a_n}^\dagger \hat{a}_{i_n} \cdots \hat{a}_{i_1} 
\end{align}
with $\hat{T}_1, \hat{T}_2, \cdots, \hat{T}_n$ being the excitation operators corresponding to single, double, and higher excitations, respectively. To make the method computationally feasible, the cluster operator is often truncated, typically including only single and double excitations, resulting in the CCSD method. The CCSD(T) method, which includes a perturbative treatment of triple excitations, is considered the gold standard in quantum chemistry and can provide highly accurate ground-state energy estimates for dynamically correlated systems. CCSD(T) scales as $O(N^7)$ and has been applied to large systems, such as a calculation on octane with 1468 basis functions using the aug-cc-pVQZ basis set with NWChem codes. The CCSD part of the calculation took 43 hours on 600 processors, and the perturbative triples took 23 hours on 1400 processors, sustaining a performance of 6.3 TFlops. Despite its somewhat favorable scaling and ability to treat dynamically correlated systems with high accuracy, CCSD(T) breaks down or yields inaccurate results for systems exhibiting static correlation (i.e., systems with multi-reference characteristics). Given the nature of the chemical systems in our computational workflow described in Section \ref{sec: Mg corrosion, sec:Nb_workflow}, we expect that many of them may exhibit static correlations.

To address static correlation, methods such as Selected Configuration Interaction (SCI)~\cite{Olsen2011,Gagliardi2007Multiconfigurational,Szalay2012Multiconfiguration} and Density Matrix Renormalization Group (DMRG)~\cite{White1992} are often employed. SCI provides a way to systematically include important configurations in the wavefunction while avoiding the combinatorial explosion of configurations. It does this by selecting a subset of configurations based on their relevance to the system's ground state. In contrast, DMRG, considered the state-of-the-art method for treating statically correlated chemical systems, relies on an approximate wavefunction ansatz known as the matrix product state (MPS). The MPS is constructed as a product of variational objects, each corresponding to an orbital within the basis. A one-site MPS is mathematically represented as:
\begin{equation}
\label{eq: one-site MPS}
|\psi \rangle = \sum_n A^{n_1} A^{n_2} \cdots A^{n_k} |n_1 n_2 \cdots n_k\rangle
\end{equation}
where $n_i$ represents the occupancy state of orbital $\phi_i$, which could be any of $|0 \rangle, |\uparrow \rangle , |\downarrow \rangle, |\uparrow \downarrow \rangle$. Each $A^{n_i}$ matrix within the MPS contains information regarding the wavefunction coefficients corresponding to the specific orbital occupancy of $\phi_i$. The $A^{n_i}$ matrices are typically $M \times M$ except for the first and last, which have dimensions $1 \times M$ and $M \times 1$, respectively. The parameter $M$, also referred to as the MPS bond dimension, dictates the number of normalized states, thus controlling both the accuracy and computational complexity of a DMRG calculation. When $M^2 \approx N_d$, where $N_d$ is the total number of possible determinants, the DMRG wavefunction becomes exact. Obtaining reliable results from SCI and DMRG requires converging the number $D$ of selected configurations and the bond dimension $B$ respectively, which is an algorithmic bottleneck. See Table \ref{tab:scaling_of_classical_methods} for a summary of the scaling for these classical approaches. 

In summary, while all of the classical methods discussed such as DFT, CCSD(T), and static correlation methods like DMRG have proven to be powerful tools in quantum chemistry, they each come with inherent limitations. DFT is fast and efficient, but it struggles with accuracy when applied to systems with strong electronic correlation. CCSD(T) can treat dynamically correlated systems but breaks down when dealing with static correlated systems.  On the other hand, methods designed to treat static correlation, such as DMRG, can provide high precision for these systems but encounter computational bottlenecks as the bond dimension must be large for complex systems, limiting scalability. In the computational workflows presented in this paper, the chemical models under consideration can exhibit both dynamically and statically correlation, thus these classical methods will encounter their respective shortcomings in these cases. Therefore, alternative approaches, such as quantum computing, are necessary to overcome these limitations and realize the proposed computational workflows.

\begin{table}[h]
    \centering
    \begin{tabular}{ccc}
        \hline\hline
        Method & Acronym & Asymptotic Scaling \\
        \hline
        Exact Diagonalization & FCI & $\binom{M}{\eta/2}$ \\
        Coupled Cluster Singles Doubles Perturbative Triples & CCSD(T) & $N^3(M-N/2)^4$ \\
        Selected Configuration Interaction & SCI & $D N^2(M-N/2)^2$ \\
        Density-Matrix Renormalization Group & DMRG & $B^3M^3 + B^2M^4$ \\
        \hline\hline
    \end{tabular}
    \caption{Summary of the asymptotic scaling for various classical computational methods. \(M\) refers to the number of spatial orbitals, \(\eta\) to the number of electrons, \(N\) to the number of basis functions, \(D\) to the number of selected configurations in SCI, and \(B\) to the bond dimension in DMRG.}
    \label{tab:scaling_of_classical_methods}
\end{table}





%%%%%%%% OLD 

% \subsection{Classical Methods for Estimating Ground-state Energies}
% \label{sec: State-of-art classical techniques}

% \subsubsection{Density functional theory}
% \label{sec: DFT}
% Given the electronic Schr\"{o}dinger Equation within the Born-Oppenheimer approximation 
% \begin{equation}
%     \label{eq: time-independent schrodinger}
%     \hat{\mathcal{H}}(r;R)|{\Psi(r;R)}\rangle =  E[\Vec{r};R]|{\Psi[r;R]}\rangle
% \end{equation}
% Where $r$ is the electronic coordinate, $R$ the nuclear coordinate that parameterizes the Schr\"{o}dinger Equation, and $\mathcal{H}$ is the Electronic Hamiltonian defined in atomic units as 
% \begin{equation}
%     \label{eq: Electronic Hamiltonian}
%     \hat{\mathcal{H}} = -\sum_i\left( \frac{\nabla_{r_i}^2}{2} + \sum_I \frac{Z_I}{|r_i - R_I|}\right) + \sum_{i<j} \frac{1}{|r_i - r_j|}
% \end{equation}
% where $Z_I$ represents the charges of the nuclei. Finding an exact solution to Equation \eqref{eq: time-independent schrodinger} is challenging because of the Coulomb repulsion between the electrons. However, the Hohenberg-Kohn theorem~\cite{Hohenberg1964Inhomogeneous} establishes a one-to-one correspondence between the ground-state electronic density and the defined Hamiltonian. Consequently, all electronic system degrees of freedom are integrated out, except for the density. This integration enables the reduction of the system size by computing the density on a three-dimensional coordinate grid, leading to significantly improved scalability compared to other methods, regardless of the number of electrons in the system. The application of this theorem extends from molecular to periodic systems, and interested readers are directed to relevant reviews for a more comprehensive explanation~\cite{Hasnip2014Density}. In principle, DFT is exact and produces the exact ground-state energy and density~\cite{Hohenberg1964Inhomogeneous}. However, in practice, it relies on approximating the exchange-correlation energy, a crucial parameter for the accuracy of DFT results. Much research has been devoted to developing such approximations, commonly termed exchange-correlation functionals. Unfortunately, there is presently no systematic approach, resulting in the proposal of hundreds of different functionals~\cite{Mardirossian2017Narbe}. The choice of functional depends strongly on the specific chemical system under study, as different bonding situations require different functional descriptions~\cite{Rappoport2005Approximate}. This is, in a way, the shortcomings associated with DFT. Therefore, while DFT is exact theoretically, practically, it is not. Some authors prefer to use the term Density Functional Approximation (DFA) to distinguish DFT from the actual calculations being executed, to highlight that the failures in these calculations are not failures of DFT itself, but rather are failures of DFAs~\cite{Becke2014Perspective}.

% The computational cost of DFT is very efficient, hence it is the most commonly use technique in a industrial setting. Early DFT codes exhibited cubic $O(N^3)$ scaling, but recent advancements have achieved linear $O(N)$ scaling. For instance, CONQUEST, a large-scale linear scaling DFT code, has been used to conduct calculations on systems of 2 million atoms using 705,024 physical cores on the Japanese Fujitsu-made K-computer~\cite{Nakata2020Large}. DFT-FE, another large-scale DFT code leveraging accurate spatially adaptive discretization strategies using high-order finite element discretization, has successfully simulated large-scale Mg dislocation systems, such as pyrIIScrewC with 6,164 Mg atoms (61,640 electrons) and pyrIIScrewC with 10,508 Mg atoms (105,080 electrons), utilizing Summit GPU nodes~\cite{Das2019Fast}.

% \subsubsection{Coupled cluster theory}

% Due to the inherent limitations of DFT, particularly in cases where strong electronic correlation effects are present, alternative systematic approaches using many-electron wavefunction theories were explored to systematically improve the accuracy in the calculation of Equation \eqref{eq: time-independent schrodinger}. One such method is coupled cluster theory. It is known as the gold standard in quantum chemistry, having been the preferred approach for over 20 years to achieve precise bond energies and molecular properties~\cite{Ramabhadran2013Extrapolation}. Coupled cluster theory is formulated as a compact wave function parametrised using an exponential functional of a cluster operator. In particular, in the second quantization framework, the coupled cluster wavefunction is given as:
% \begin{equation}
% \label{eq: Coupled Cluster}
% |\psi_{\text{CC}} \rangle = e^{\hat{T}}|\Phi_0\rangle = \sum_{i} \frac{1}{i!} (\hat{T})^n |\Phi_0\rangle
% \end{equation}
% where 
% \begin{align}
% \hat{T} &= \hat{T}_1 + \hat{T}_2 + \ldots + \hat{T}_n \\
% &=  \sum_{ai} t_i^a \hat{a}^\dagger_a \hat{a}_i 
% + \frac{1}{4} \sum_{abij} t_{ij}^{ab} \hat{a}^\dagger_a \hat{a}^\dagger_b \hat{a}_j \hat{a}_i 
% + \cdots + \frac{1}{ (n!)^2} \sum_{i_1, \cdots, i_n, a_1, \cdots, a_n} t_{i_1 \cdots i_n}^{a_1 \cdots a_n} \hat{a}_{a_1}^\dagger \cdots \hat{a}_{a_n}^\dagger \hat{a}_{i_n} \cdots \hat{a}_{i_1}
% \end{align}
% with $\hat{T}_1, \hat{T}_2, \cdots, \hat{T}_n$ being the excitation operators corresponding to single, double, and higher excitations, respectively. Note that the subscript refers to the number of excited electrons. $|\Phi_0\rangle$ is the Hartree-Fock state. $\hat{a}_i^\dagger$ and $\hat{a}_i$ are the creation and annhihilators operators corresponding to the $i$ orbital, respectively. The expansion coefficients $t_i$ are called the amplitudes. In practice, one needs to truncate $\hat{T}$ to consider only single and double excitations to make the computation feasible. In this scenario, where only single and double excitations (CCSD) are considered, the computational time scales as $O(N^6)$, where $N$ is the number of basis functions (orbitals). It should be noted that under the tensor hypercontraction (THC) framework, CCSD has the scaling of $O(N^4)$. In practice, CCSD(T), CCSD with perturbative triples, is the largest type of CC calculation one can perform. CCSD(T) scales as $O(N^7)$, (or $O(N^5)$ under THC framework) and it's the gold standard for computational chemistry. One of the largest CCSD(T) calculations was performed on octane with 1468 basis functions using the aug-cc-pVQZ basis set with NWChem codes. The CCSD part of the calculation took 43 hours on 600 processors, and the perturbative triples took 23 hours on 1400 processors, sustaining a performance of 6.3 TFlops. 


% \subsubsection{Quantum Monte-Carlo}
% Quantum Monte Carlo (QMC) methods are a family of methods aimed at studying complex systems at a reduced cost. Among these methods is a particular subset known as Variational Monte Carlo (VMC). These techniques involve the direct application of Monte Carlo integration and are specifically tailored to approximate the ground state of a quantum system by minimizing the energy functional. More specifically, it relies on minimizing the energy functional $E[\psi_T(\mathbf{\theta}) ]$

% \begin{equation}
%     E[\psi_T(\mathbf{\theta}) ] = \frac{\int \psi_T^*(\mathbf{r}, \mathbf{\theta}) H \psi_T(\mathbf{r}, \mathbf{\theta}) d\mathbf{r} }{\int \psi_T^*(\mathbf{r}, \mathbf{\theta}) \psi_T(\mathbf{r}, \mathbf{\theta}) d\mathbf{r}  } = \frac{\int |\psi_T(\mathbf{r}, \mathbf{\theta})|^2 \frac{H \psi_T(\mathbf{r}, \mathbf{\theta})}{\psi_T(\mathbf{r}, \mathbf{\theta})} d\mathbf{r}  }{ \int |\psi_T(\mathbf{r}, \mathbf{\theta})|^2 d\mathbf{r}  }
% \end{equation}
% where $H$ is the electronic Hamiltonian described in Equation \eqref{eq: Electronic Hamiltonian}, and $\psi_T(\mathbf{r}, \mathbf{\theta})$ is a general wave-function consisting of $N_e$ particles located at positions $\mathbf{r}= (r_1, r_2, \cdots, r_{N_e})$ depending on some arbitrary parameters $\mathbf{\theta}$. $E_L(\mathbf{r}) = \frac{H \psi_T(\mathbf{r}, \mathbf{\theta})}{\psi_T(\mathbf{r}, \mathbf{\theta})}$ is known as the ``local energy''. To optimize the wavefunction, $\psi_T(\mathbf{r},\mathbf{\theta})$, stochastic optimization algorithms such as the Metropolis algorithm can be used to sample configurations of the system's coordinate according its  probability. The trail wavefunction, $\psi_T(\mathbf{\theta})$, is a critical component in the success and cost of the algorithm. Typically, the computational cost of running VMC is around $O(N_e^3)$ to $O(N_e^4)$~\cite{Williams2020Direct}, thus exhibiting similar scaling as CCSD.



% \subsubsection{Multiconfigurational Quantum Chemistry and Density matrix renormalization group}
% \label{sec: DMRG}
% Multi-reference chemistry methods such as complete active space configuration interaction (CASCI) and self-consistent field (CASSCF) are used to address the issue of static correlation while maintaining some computational tractability. In-depth reviews of these methods are provided elsewhere~\cite{Olsen2011,Gagliardi2007Multiconfigurational,Szalay2012Multiconfiguration}. In general, these methods aim to expand the wavefunction to include many electronic configurations for a region of the molecule expected to have significant static correlation contributions to energy while freezing the orbitals outside of that space. This is akin to solving FCI for a subset of orbitals embedded within a single-reference method. While these methods are improvements on solving the \textit{whole} problem, active orbitals must be selected carefully to minimize the issue of scaling within the active space. To date, the largest-size simulations on exascale computing hardware have reached up to 20 orbitals for CASSCF and 22 orbitals for CASCI simulations~\cite{Vogiatzis2017}. 

% The density matrix renormalization group (DMRG) is a method to increase the classical capacity for multiconfigurational methods~\cite{White1992}. It  is founded upon an approximate wavefunction ansatz known as the matrix product state (MPS), constructed as a product of variational objects for each orbital within the basis. A one-site MPS is mathematically represented as:
% \begin{equation}
% \label{eq: one-site MPS}
% |\psi \rangle = \sum_n A^{n_1} A^{n_2} \cdots A^{n_k} |n_1 n_2 \cdots n_k\rangle
% \end{equation}
% where $n_i$ represents the occupancy state of orbital $\phi_i$, which could be any of $|0 \rangle, |\uparrow \rangle , |\downarrow \rangle, |\uparrow \downarrow \rangle$. Each $A^{n_i}$ matrix within the MPS contains information regarding the wavefunction coefficients corresponding to the specific orbital occupancy of $\phi_i$. The $A^{n_i}$ matrices are typically $M \times M$ except for the first and last, which have dimensions $1 \times M$ and $M \times 1$, respectively. The parameter $M$, also referred to as the MPS bond dimension, dictates the number of normalized states, thus controlling both the accuracy and computational complexity of a DMRG calculation. When $M^2 \approx N_d$, where $N_d$ is the total number of possible determinants, the DMRG wavefunction becomes exact. Thus, varying $M$ allows for a much cheaper computational cost, and in practice, for $M$ in the range of one to ten thousand can be used to achieve chemical accuracy. This scalability allows DMRG to be applied to large active spaces with more than 50 orbitals~\cite{Olivares2015ab}. This is much larger than conventional active space methods such as CASSCF~\cite{Chan2004State}.

